Search Trajectories Networks of Multiobjective Evolutionary Algorithms

Understanding the search dynamics of multiobjective evolutionary algorithms (MOEAs) is still an open problem. This paper extends a recent network-based tool, search trajectory networks (STNs), to model the behavior of MOEAs. Our approach uses the idea of decomposition, where a multiobjective problem is transformed into several single-objective problems. We show that STNs can be used to model and distinguish the search behavior of two popular multiobjective algorithms, MOEA/D and NSGA-II, using 10 continuous benchmark problems with 2 and 3 objectives. Our findings suggest that we can improve our understanding of MOEAs using STNs for algorithm analysis.

==> files/nsga2.tex <==

\begin{algorithm}[htbp]
\Yuri{I need to check this code}
\caption{Non-dominated Sorting}\label{alg:non_dominated_sorting}
\begin{algorithmic}[1]
\For{individual $\mathbf{x}$ in population $X$}
    \State Set $S_{\mathbf{x}} = \emptyset$ and $n_{\mathbf{x}} = 0$;
    \For{individual $\mathbf{y}$ in population $X$}
        \If{$\mathbf{x} \prec \mathbf{y}$}
            \State Update $S_{\mathbf{x}} = S_{\mathbf{x}} \bigcup \{ \mathbf{y} \}$;
        \ElsIf{$\mathbf{y} \prec \mathbf{x}$}
            \State Update $n_{\mathbf{x}} = n_{\mathbf{x}} + 1$;
        \EndIf
    \EndFor
    \If{$n_{\mathbf{x}}$ = 0}
        \State Set $\mathbf{x}_{rank} = 1$ and update $R_{1} = R_{1} \bigcup \{ \mathbf{x} \}$;
    \EndIf
\EndFor
\State $i = 1$;
\While{$R_i \neq \emptyset$}
    \State Set $Q=\emptyset$;
    \For{individual $\mathbf{x}$ in $R_i$}
        \For{individual $\mathbf{y}$ in $S_{\mathbf{x}}$}
            \State Update $n_{\mathbf{y}} = n_{\mathbf{y}} - 1$;
            \If{$n_{\mathbf{y}} = 0$}
                \State Set $\mathbf{y}_{rank} = i + 1$ and update $Q = Q \bigcup \{ \mathbf{y} \}$;
            \EndIf
        \EndFor
    \EndFor
    \State Update $i = i + 1$;
    \State Set $R_i = Q$;
\EndWhile
\end{algorithmic}
\end{algorithm}

